Improving Reasoning Performance in Large Language Models via Representation Engineering

Recent advancements in large language models (LLMs) have resulted in increasingly anthropomorphic language concerning the ability of LLMs to reason. Whether reasoning in LLMs should be understood to be inherently different is, however, widely debated. We propose utilizing a representation engineering approach wherein model activations are read from the residual stream of an LLM when processing a reasoning task. The activations are used to derive a control vector that is applied to the model as an inference-time intervention, modulating the representational space of the model, to improve performance on the specified task. We publish the code for deriving control vectors and analyzing model representations. The method allows us to improve performance on reasoning benchmarks and assess how control vectors influence the final logit distribution of a model via metrics such as KL divergence and entropy. We apply control vectors to Mistral-7B-Instruct and a range of Pythia models on an inductive, a deductive and mathematical reasoning task. We show that an LLM can, to a certain degree, be controlled to improve its perceived reasoning ability by modulating activations. The intervention is dependent upon the ability to reliably extract the model's typical state when correctly solving a task. Our results suggest that reasoning performance can be modulated in the same manner as other information-processing tasks performed by LLMs and demonstrate that we are capable of improving performance on specific tasks via a simple intervention on the residual stream with no additional training.

==> tex/A1.tex <==
As can be gathered from equation \ref{equation:control-vector} any control vector will have a norm that is equivalent to the average of the hidden dimension activations at a given layer of the model. For the contrastive pairs (equation \ref{equation:contrast-control-vector}) it will be equivalent to the norm one gets when subtracting the "opposite" state from the "desired" state. This is however not the case for the control vector based on a PCA, because a standard PCA implementation scales the output vector to have an L2 norm of 1. We cannot know the exact size of $||H_{\ell}||$ as this is dependent on the learned parameters $\gamma$ and $\beta$ of the \LN function. Assuming $\gamma = 1$ and $\beta = 0$, which are the usual initial values \citep{baLayer2016}, a rough estimate of the norm of the hidden dimension, d, is $||H_{\ell}|| = \sqrt{d}$, the value however varies a lot dependent on the model and between layers. We therefore scale the PCA control vectors by $||H_{\ell}||$ of the training data to allow for a more direct comparison between the control vector methods. As indicated by figure \ref{fig:cv-norms} we get identical norms for the two methods, while the actual control vectors are different.

\begin{figure}[htbp]
    \centering
    \subfloat[Reading Contrast CV - Pythia 1.4b]{%
        \includegraphics[width=0.49\textwidth]{plots/RC-NORMS_pythia-1.4b.png}%
        \label{fig:subfig1}%
    }%
    \hfill
    \subfloat[Reading Contrast CV - Pythia 2.8b]{%
        \includegraphics[width=0.49\textwidth]{plots/RC-NORMS_pythia-2.8b.png}%
        \label{fig:subfig2}%
    }%
    \hfill
    \subfloat[PCA Contrast CV - Pythia 1.4b]{%
        \includegraphics[width=0.49\textwidth]{plots/PCA-NORMS_pythia-1.4b.png}%
        \label{fig:subfig3}%
    }%
    \hfill
    \subfloat[PCA Contrast CV - Pythia 2.8b]{%
        \includegraphics[width=0.49\textwidth]{plots/PCA-NORMS_pythia-2.8b.png}%
        \label{fig:subfig4}%
    }
    \caption{Control Vector Norms}
    \label{fig:cv-norms}
\end{figure}
